Distributed estimation and control of node centrality in undirected asymmetric networks

Measures of node centrality that describe the importance of a node within a network are crucial for understanding the behavior of social networks and graphs. In this paper, we address the problems of distributed estimation and control of node centrality in undirected graphs with asymmetric weight values. In particular, we focus our attention on $\alpha$-centrality, which can be seen as a generalization of eigenvector centrality. In this setting, we first consider a distributed protocol where agents compute their $\alpha$-centrality, focusing on the convergence properties of the method; then, we combine the estimation method with a consensus algorithm to achieve a consensus value weighted by the influence of each node in the network. Finally, we formulate an $\alpha$-centrality control problem which is naturally decoupled and, thus, suitable for a distributed setting and we apply this formulation to protect the most valuable nodes in a network against a targeted attack, by making every node in the network equally important in terms of {\alpha}-centrality. Simulations results are provided to corroborate the theoretical findings.

==> OptimizationOLD.tex <==
\section{Distributed Control of Node $\alpha$-Centrality}
\label{sec:control}
There are other applications involving networks, where rather than estimating the current centrality measure of each node, we are interested in \emph{controlling} its value.
This sections discusses an optimization problem that can be solved by standard methods to perform minimum variations on the influence matrix to achieve this objective in finite time with only one round of communication.
%In this section we present a distributed algorithm that allows each agent in the network to perform minimum variations on the influence matrix to achieve this objective in finite time with only one round of communication.

In particular, let $\bm\rho_\alpha^*$ be the desired $\alpha$-centrality vector for a given graph $\mathcal{G}$ with initial influence matrix $\mathbf{W}$ and let $\overline{\mathbf{W}}\in\mathbb{A}_G$ and $\underline{\mathbf{W}}\in\mathbb{A}_G$ with $\overline{\mathbf{W}}\geq \mathbf{W}\geq \underline{\mathbf{W}}$.
Similarly to the definition of $w_{ij}$, we denote by $x_{ij}$ the amount of variation applied on the influence of agent $j$'s information for agent $i$, and $\mathbf{X}=[x_{ij}]$ the matrix containing all the changes in the original influence matrix.
Our goal in this section is then to
find the matrix $\mathbf{X}^*\in \mathbb{A}_{\mathcal{G}}$ that solves
\begin{equation}
\label{prob:convexproblem0}
\begin{aligned}
& \underset{\mathbf{X}\in \mathbb{A}_{\mathcal{G}}}{\min}
& &\dfrac{1}{2}\|\mathbf{X}\|_F^2 \\
& \text{subject to}
& & \mathbf{W}+\mathbf{X} \leq \overline{\mathbf{W}} \\
& & &\mathbf{W}+\mathbf{X} \geq \underline{\mathbf{W}}\\
& & & (I_n-\alpha(\mathbf{W} + \mathbf{X})^T)\bm\rho_\alpha^* = \mathbf{z}.
%\\& & & \textcolor{black}{(\mathbf{W} + \mathbf{X})^T\bm\rho_\alpha^* = \dfrac{\bm\rho_\alpha^*-\mathbf{z}}{\alpha}.}
\end{aligned}\end{equation}
%\end{problem} 
The above optimization problem represents that we want minimum effort variation on the matrix $\mathbf{W}$; in this view, we are interested in scenarios where the nodes aim at  slightly modifying how their neighbors perceive their importance in the network while changing the $\alpha$-centrality to the desired value.
The first two constraints are included to model the fact that every influence value cannot change more than an arbitrary amount, encoded by the matrices $\overline{\mathbf{W}}$ and $\underline{\mathbf{W}}$.
The last constraint in Eq.~\eqref{prob:convexproblem0} imposes that the new influence matrix, $\mathbf{W}+\mathbf{X}$, has to yield the desired centrality value.

Let us now provide a necessary and sufficient optimality condition for Problem~\eqref{prob:convexproblem0}, under the assumptions given in Proposition~\ref{prop:feasibility}.
To this end, let us introduce some useful notation.
Specifically, consider a vector \mbox{${\bm \lambda}=[\lambda_1,\ldots,\lambda_n]^T$} and let $\mathbf{P}({\bm \lambda})\in \mathbb{A}_{\mathcal{G}}$ be the $n\times n$ matrix such that
\begin{equation}
\label{eq:optimalW}
p_{ij}({\bm \lambda})= 
\begin{cases}
sat\left(w_{ij}-\lambda_j\rho^*_{\alpha i},\underline w_{ij},\overline w_{ij}\right),&\mbox{ if } j\in \widehat{\mathcal{N}}_i\\
%%(i,j)\in \mathcal{E} \mbox{ or } i=j\\
0&\mbox{ otherwise.}
\end{cases}
\end{equation}
Moreover, let us define $f:\mathbb{R}^n \rightarrow \mathbb{R}^n$ as
\begin{equation}
f({\bm \lambda})=\mathbf{P}^T({\bm \lambda})\bm\rho_\alpha^*-\dfrac{\bm\rho_\alpha^*-\mathbf{z}}{\alpha}
\end{equation}

Notably, the idea of solving a distributed optimization problem with minimum effort has been applied also in \cite{oliva2019distributed}, where an optimal weight balancing problem is solved by first providing a necessary and sufficient optimality condition and then by resorting to dynamical equations that asymptotically converges to an optimal solution. In this paper we also provide a necessary and sufficient optimality condition, but we develop a finite time algorithm to compute it, which relies on a single communication round, while all further computations are performed locally at each agent.



In the further developments of this section, we assume that the problem in Eq.~\eqref{prob:convexproblem0} admits at least one feasible solution. To this end, it is convenient to provide a feasibility condition, as done in the next proposition.
\textcolor{black}{
\begin{proposition}
\label{prop:feasibility}
Suppose $\underline{\mathbf{W}}\geq 0_{n\times n}$ and $\bm\rho_\alpha^*\geq \mathbf{z}$. The problem in Eq.~\eqref{prob:convexproblem0} admits a feasible solution if and only if it holds
\begin{equation}
\label{eq:feasibility}
\begin{cases}
(I_n-\alpha\overline{\mathbf{W}}^T)\rho_\alpha^*\leq  \mathbf{z}
\\
(I_n-\alpha\underline{\mathbf{W}}^T)\rho_\alpha^*\geq  \mathbf{z}
\end{cases}
\end{equation}
\end{proposition}
\begin{proof}
%
The equation
$$
(I_n-\alpha(\mathbf{W} + \mathbf{X})^T)\bm\rho_\alpha^* = \mathbf{z}
$$
is equivalent to
$$
(\mathbf{W} + \mathbf{X})^T\bm\rho_\alpha^*=\dfrac{\rho_\alpha^*-\mathbf{z}}{\alpha}.
$$
Since $\underline{\mathbf{W}}\geq 0_{n\times n}$, we have that any admissible $\mathbf{X}$ satisfies
$$
\mathbf{W} + \mathbf{X}\geq 0_{n\times n},
$$
i.e., the entries of $\mathbf{W} + \mathbf{X}$ are nonnegative.
Therefore, since also the entries of $\bm\rho_\alpha^*$ are nonnegative, it holds
$$
\underline{\mathbf{W}}\rho_\alpha^*\leq (\mathbf{W} + \mathbf{X})^T)\bm\rho_\alpha^* \leq \overline{\mathbf{W}}\rho_\alpha^*,
$$
and thus, the problem admits a feasible solution if and only if
$$
\begin{cases}
\dfrac{\rho_\alpha^*-\mathbf{z}}{\alpha}\leq\overline{\mathbf{W}}^T\bm\rho_\alpha^*\\
\dfrac{\rho_\alpha^*-\mathbf{z}}{\alpha}\geq\underline{\mathbf{W}}^T\bm\rho_\alpha^*
\end{cases}
$$
which is equivalent to Eq.~\eqref{eq:feasibility}. The proof is complete.
\end{proof}
}
%\textcolor{black}{The objective function represents the fact we want minimum effort variation of W, the first set of constraints means... Complete the description.}
%\textcolor{black}{NOTE: the $*$ in $\rho_\alpha^*$ can be confusing since I am using $X^*$ to denote the optimal $X$. I am open to changes if needed.}

%\textcolor{black}{Add brief description of the problem.}
%\begin{problem}%[Proximity-Constrained Non-Exclusive Coverage]
%\label{prob:ourproblem}

% \mbox{$\mathcal{G}=\{\mathcal{V},\mathcal{E}\}$}  be a connected undirected graph with $n$ nodes, and let a  matrix $\mathbf{W}\in\mathbb{A}_{\mathcal{G}}$ a scalar $\alpha>0$  and vectors $\bm\rho_\alpha^*\in\mathbb{R}^n_{\geq 0}$  and $\mathbf{z}\in\mathbb{R}^n_{\geq 0}$. (\textcolor{black}{check range of existence of the constants; are they all positive, nonnegative, etc.?})
%Moreover, let $\underline{\mathbf{W}}\in\mathbb{A}_{\mathcal{G}}$ and $\overline{\mathbf{W}}\in\mathbb{A}_{\mathcal{G}}$ be such that $\underline{\mathbf{W}}\leq\mathbf{W}\leq\overline{\mathbf{W}}$ and $\underline{\mathbf{W}}<\overline{\mathbf{W}}$.




%\begin{remark}
%Notice that, since $\underline{\mathbf{W}}\leq\mathbf{W}\leq\overline{\mathbf{W}}$ and $\underline{\mathbf{W}}<\overline{\mathbf{W}}$, we have that Problem~\eqref{prob:convexproblem0} always admits a feasible solution  $\mathbf{X}=\mathbf{0}_{n\times n}$.
%\textcolor{black}{Is it correct? please check.}
%\end{remark}
%\red{I don't think this is correct}


\begin{theorem}
\label{firstorderproblema}
Under the assumptions given in Proposition~\ref{prop:feasibility},  the problem in Eq.~\eqref{prob:convexproblem0} admits a global minimum $\mathbf{X}^*\in \mathbb{A}_{\mathcal{G}}$ in the form
\begin{equation}
\label{eq:optimalX}
\mathbf{X}^*=\mathbf{P}({\bm \lambda}^*)-\mathbf{W},
\end{equation}
where the vector ${\bm \lambda}^*\in\mathbb{R}^n$  satisfies
\begin{equation}
\label{eq:optimallambda}
f({\bm \lambda}^*)={\bm 0}_n.
%\left(\alpha\mathbf{Z}^T({\bm \lambda}^*)-\mathbf{I}_n\right)\bm\rho_\alpha^*+\mathbf{z}=\mathbf{0}_n.
\end{equation}
\end{theorem}
\begin{proof}
By construction, the objective function of Problem~\eqref{prob:convexproblem0} is differentiable and convex, while all its constraints are linear; moreover, by assumption, Problem~\eqref{prob:convexproblem0} is feasible. Therefore the KKT necessary and sufficient conditions in Theorem~\ref{theoKKT} apply.

Let us consider Lagrange multipliers \mbox{${\bm \Phi}\in \mathbb{A}_{\mathcal{G}}$}, \mbox{${\bm \Psi}\in \mathbb{A}_{\mathcal{G}}$} and \mbox{${\bm \lambda}\in \mathbb{R}^{n}$},
that correspond to the first, second and third sets of constraints in Eq.~\eqref{prob:convexproblem0}, respectively. 
%
The Lagrange function $\mathcal{L}(\mathbf{ X},{\bm \Phi},{\bm \Psi},{\bm \lambda})$ associated to the Problem in Eq.~\eqref{prob:convexproblem0}~is
$$
\begin{aligned}
&\mathscr{L}(\cdot)=\dfrac{1}{2}\sum_{(i,j)\in \mathcal{E}}x_{ij}^2
+\sum_{(i,j)\in \mathcal{E}} { \phi}_{ij}(w_{ij}+x_{ij}-\overline{w}_{ij})\\
&+\sum_{(i,j)\in \mathcal{E}} { \psi}_{ij}(-w_{ij}-x_{ij}+\underline w_{ij})\\
&+\sum_{i=1}^n\lambda_i\left(\displaystyle\sum_{j\in \widehat{\mathcal{N}}_i}^n (w_{ji}+x_{ij})\rho^*_{\alpha j}-\frac{1}{\alpha}\rho^*_{\alpha i}+\frac{1}{\alpha}z_i\right).
\end{aligned}
$$
%
By Theorem~\ref{theoKKT}, $\mathbf{X}^*$ is the global minimum if and only if there are ${\bm \Phi}^*\in \mathbb{A}_{\mathcal{G}}$, ${\bm \Psi}^*\in \mathbb{A}_{\mathcal{G}}$ and ${\bm \lambda}^*\in \mathbb{R}^{n}$ such that the following conditions hold true for all $(i,j)\in \mathcal{E}$
\begin{equation}
\label{KKTcond:1}
\frac{\partial \mathcal{L}(\cdot)}{\partial X_{ij}}\Big|_{\mathbf{X}=\mathbf{X}^*,{\bm \Phi}={\bm \Phi}^*,{\bm \Psi}={\bm \Psi}^*,{\bm \lambda}={\bm \lambda}^*}=0,
\end{equation}
\begin{equation}
\label{KKTcond:2}
w_{ij}+x_{ij}^*\geq\underline w_{ij},
\end{equation}
\begin{equation}
\label{KKTcond:3}
w_{ij}+x_{ij}^*\leq \overline w_{ij},
\end{equation}
\begin{equation}
\label{KKTcond:4}
(I_n-\alpha(\mathbf{W} + \mathbf{X})^T)\bm\rho_\alpha^* = \mathbf{z}
\end{equation}
\begin{equation}
\label{KKTcond:5}
{\phi}^*_{ij}(w_{ij}+x_{ij}^*-\overline w_{ij})=0,
\end{equation}
\begin{equation}
\label{KKTcond:6}
{\psi}^*_{ij}(w_{ij}+x_{ij}^*-\underline w_{ij})=0,
\end{equation}
\begin{equation}
\label{KKTcond:7}
{\psi}^*_{ij}\geq0,
\end{equation}
\begin{equation}
\label{KKTcond:8}
{\phi}^*_{ij}\geq0.
\end{equation}
In particular, the condition in Eq.~\eqref{KKTcond:1} corresponds to
\begin{equation}
\label{eq:primasoluzionediXstar}
\begin{aligned}
x^*_{ij}={ \psi}^*_{ij}-{ \phi}^*_{ij}-\lambda^*_j\rho^*_{\alpha i},
\end{aligned}
\end{equation}
where we refer to the $i$-th component of the vector ${\bm \rho}_\alpha$ as $\rho^*_{\alpha i}$.
At this point, we plug Eq.~\eqref{eq:primasoluzionediXstar} into Eqs.~\eqref{KKTcond:7}~and~\eqref{KKTcond:8}, and we obtain, respectively,
\begin{equation}
\label{eq:primasoluzionediPhi}
{\phi}^*_{ij}(w_{ij}+{ \psi}^*_{ij}-{ \phi}^*_{ij}-\lambda^*_j\rho^*_{\alpha i}-\overline w_{ij})=0
\end{equation}
and
\begin{equation}
\label{eq:primasoluzionediPsi}
{\psi}^*_{ij}(w_{ij}+{ \psi}^*_{ij}-{ \phi}^*_{ij}-\lambda^*_j\rho^*_{\alpha i}-\underline w_{ij})=0.
\end{equation}
We observe that, when ${\phi}^*_{ij}>0$ it must hold \mbox{$w_{ij}+x_{ij}=\overline w_{ij}$} and thus \mbox{$w_{ij}+x_{ij}\neq\underline w_{ij}$}, which implies that $\psi^*_{ij}=0$; as a consequence, when ${\phi}^*_{ij}>0$, by Eq.~\eqref{eq:primasoluzionediPhi}  we have that 
$${\phi}^*_{ij}=w_{ij}-\lambda^*_j\rho^*_{\alpha i}-\overline w_{ij}.$$
Since ${\phi}^*_{ij}\geq 0$, we conclude that 
$${\phi}^*_{ij}=\max\{0,w_{ij}-\lambda^*_j\rho^*_{\alpha i}-\overline w_{ij}\}.$$
With a similar reasoning, we have that 
\begin{equation*}
\psi^*_{ij}=\max\{0,-w_{ij}+\lambda^*_j\rho^*_{\alpha i}+\underline w_{ij}\}.
\end{equation*}
Therefore, it holds
\begin{equation*}
{\psi}^*_{ij}-{\phi}^*_{ij}=
\begin{cases}
-w_{ij}+\lambda^*_j\rho^*_{\alpha i}+\underline w_{ij}& \mbox{ if } w_{ij}-\lambda^*_j\rho^*_{\alpha i}<\underline w_{ij}\\
-w_{ij}+\lambda^*_j\rho^*_{\alpha i}+\overline w_{ij}& \mbox{ if } w_{ij}-\lambda^*_j\rho^*_{\alpha i}>\overline w_{ij}\\
0& \mbox{ otherwise}
%\mbox{ if } \underline w_{ij}<w_{ij}-\lambda^*_j\rho^*_{\alpha i}<\overline w_{ij}
\end{cases}
\end{equation*}
The above expression is equivalent to
\begin{equation*}
\begin{aligned}
{\psi}^*_{ij}-{\phi}^*_{ij}&=-w_{ij}+\lambda^*_j\rho^*_{\alpha i}+sat(w_{ij}-\lambda^*_j\rho^*_{\alpha i},\underline w_{ij},\overline w_{ij})\\
&=-w_{ij}+\lambda^*_j\rho^*_{\alpha i}+p_{ij}({\bm \lambda}^*).
\end{aligned}
\end{equation*}
Plugging the above equation into Eq.~\eqref{eq:primasoluzionediXstar}, we get
\begin{equation}
\label{eq:pippotrue}
x^*_{ij}=p_{ij}({\bm \lambda}^*)-w_{ij}\quad\Rightarrow \quad\mathbf{X}^*=\mathbf{P}({\bm \lambda}^*)-\mathbf{W}.
\end{equation}
Plugging Eq.~\eqref{eq:pippotrue} in Eq.~\eqref{KKTcond:4}, we conclude that 
$$
\left(I_n-\alpha\mathbf{P}^T({\bm \lambda}^*)\right)\bm\rho_\alpha^*=\mathbf{z}
$$
by which Eq.~\eqref{eq:optimallambda} follows.
This completes our proof.
\end{proof}

%\red{Explain that then we transform the original problem into an easier one of computing the Lagrange multipliers}


\subsection{Finite-time Computation of the Optimal Solution}
%\begin{remark}
%\label{rem:remarkflocal}
In order to calculate the global minimum of Problem~\eqref{prob:convexproblem0}, we seek ${\bm \lambda}^*\in\mathbb{R}^n$ that satisfies $f({\bm \lambda}^*)=\mathbf{0}_n$.
Specifically, for all $i\in\{1,\ldots,n\}$, we have that
\begin{equation}
\label{eq:fi}
f_i({\bm \lambda}^*)= \sum_{j\in\widehat{\mathcal{N}}_i} 
sat\left(w_{ji}-\lambda_i^*\rho^*_{\alpha j},\underline w_{ji},\overline w_{ji}\right)\rho^*_{\alpha j}-\dfrac{1}{\alpha}(\rho^*_{\alpha i}-z_i).
\end{equation}
From the above equation, it is evident that $f_i({\bm \lambda}^*)$ is indeed a function of just the $i$-th component $\lambda^*_i$, i.e., $f_i({\bm \lambda}^*)=f_i({ \lambda}^*_i)$.
As a consequence, we have that if each agent knows the coefficients $w_{ji},\overline w_{ji},\underline w_{ji},\rho^*_{\alpha j}$ associated to its neighbors--such an information can be obtained via a single communication round--it is able to compute its own $\lambda^*_i$ without further communication.
In other words, the problem of finding the optimal ${\bm \lambda}^*$ can be decomposed into $n$ independent tasks that can be solved locally (except for one preliminary  communication round) at each agent.
%\end{remark}

%Gabriele, with one round of communication
We exploit this idea %discussed in Remark~\ref{rem:remarkflocal} 
to develop an algorithm to let each agent~$i$ independently compute its associated ${ \lambda}^*_i$ and the terms $p_{ji}(\cdot)$. This computation is done in finite time and with just one communication round, in which the agents share information with their neighbors in order to know the entries $w_{ji},\overline w_{ji},\underline w_{ji}$.
Notice that, if needed, each agent~$i$ is able to obtain the terms $p_{ij}(\cdot)$ from its neighbors via an additional communication round at the end of the procedure.




Within the proposed algorithm, we aim at finding $\lambda^*_i$ by decomposing $\widehat{\mathcal{N}}_i$ 
%(we recall that $\widehat{\mathcal{N}}_i={\mathcal{N}}_i\cup\{v_i\}$) 
into three mutually exclusive and possibly empty sets
$$\widehat{\mathcal{N}}_i^{\leftrightarrow}=\left\{j\in\widehat{\mathcal{N}}_i\,\,\Big|\, w_{ji}-\lambda_i^*\rho^*_{\alpha j}\in(\underline w_{ji},\overline w_{ji})\right\},$$
$$\widehat{\mathcal{N}}_i^{\downarrow}=\left\{j\in\widehat{\mathcal{N}}_i\,\,\Big|\, w_{ji}-\lambda_i^*\rho^*_{\alpha j}\leq\underline w_{ji}\right\},$$
and
$$\widehat{\mathcal{N}}_i^{\uparrow}=\left\{j\in\widehat{\mathcal{N}}_i\,\,\Big|\, w_{ji}-\lambda_i^*\rho^*_{\alpha j}\geq\overline w_{ji}\right\}.$$
Notice that $\widehat{\mathcal{N}}_i^{\leftrightarrow}$ %\textcolor{black}{(should we use $\widehat{\mathcal{N}}_i$ or $\widehat{\mathcal{N}}_i$? I used the first, but I have seen also the latter around. )}
is the subset of $\widehat{\mathcal{N}}_i$ for which the argument $w_{ji}-\lambda_i^*\rho^*_{\alpha j}$ of the saturation function that defines $p_{ij}(\cdot)$ belongs to the interval $(\underline w_{ji},\overline w_{ji})$, while $\widehat{\mathcal{N}}_i^{\downarrow}$,  $\widehat{\mathcal{N}}_i^{\uparrow}$ represent the subsets of $\widehat{\mathcal{N}}_i$ for which the saturation saturates below and above, respectively.

Let us define  the following Boolean variables for  all $j\in \widehat{\mathcal{N}}_i$
$$
x^{\leftrightarrow}_j=
\begin{cases}
1& \mbox{ if }  j\in \widehat{\mathcal{N}}_i^{\leftrightarrow}\\
0& \mbox{ otherwise},
\end{cases}
$$
$$
x^{\downarrow}_j=
\begin{cases}
1& \mbox{ if }  j\in \widehat{\mathcal{N}}_i^{\downarrow}\\
0& \mbox{ otherwise},
\end{cases}
$$
$$
x^{\uparrow}_j=
\begin{cases}
1& \mbox{ if }  j\in \widehat{\mathcal{N}}_i^{\uparrow}\\
0& \mbox{ otherwise}.
\end{cases}
$$

Considering these definitions, our goal is to compute the optimal $\lambda_i^*$ 
%we now introduce the following problem.
%\begin{problem}%[Proximity-Constrained Non-Exclusive Coverage]
%\label{prob:satisfaction}
%Let the assumptions of Problem~\eqref{prob:convexproblem0} hold true.
%Find $\lambda^*_i\in \mathbb{R}$ 
and $x^{\leftrightarrow}_j,x^{\downarrow}_j,x^{\uparrow}_j \in \{0,1\}$ for all $j\in \widehat{\mathcal{N}}_i$ that satisfy the following constraints
\begin{subequations}
\label{prob:constraints}
    \begin{align}
    \lambda^*_i \displaystyle\sum_{j\in \widehat{\mathcal{N}}_i}x^{\leftrightarrow}_j(\rho^*_{\alpha_j})^2=\displaystyle
    \sum_{j\in\widehat{\mathcal{N}}_i}&\left(x^{\leftrightarrow}_jw_{ji}+x^{\downarrow}_j\underline w_{ji}+x^{\uparrow}_j\overline w_{ji}\right)\rho^*_{\alpha j} \nonumber\\
    \label{prob:constraint1}
    &+\frac{z_i-\rho^*_{\alpha i}}{\alpha},\\
    \label{prob:constraint2}
    x^{\leftrightarrow}_j+x^{\downarrow}_j+x^{\uparrow}_j=1&,\quad \forall j\in \widehat{\mathcal{N}}_i,\\
    \label{prob:constraint3}
    w_{ji}-\lambda^*_i \rho^*_{\alpha j}\in(\underline w_{ji},\overline w_{ji})&,\quad \forall j\in \widehat{\mathcal{N}}_i\,|\, x^{\leftrightarrow}_j=1,\\
    \label{prob:constraint4}
    w_{ji}-\lambda^*_i \rho^*_{\alpha j}\leq \underline w_{ji}&,\quad \forall j\in \widehat{\mathcal{N}}_i\,|\, x^{\downarrow}_j=1,\\
    \label{prob:constraint5}
    w_{ji}-\lambda^*_i \rho^*_{\alpha j}\geq \overline w_{ji}&,\quad \forall j\in \widehat{\mathcal{N}}_i\,|\, x^{\uparrow}_j=1.
    \end{align}
\end{subequations}


% \begin{equation}
% \label{prob:constraint1}
% \begin{aligned}
% \lambda^*_i \displaystyle\sum_{j\in \widehat{\mathcal{N}}_i}x^{\leftrightarrow}_j\rho_{\alpha^*j}^2&=\displaystyle
% \sum_{j\in\widehat{\mathcal{N}}_i}\left(x^{\leftrightarrow}_jw_{ji}+x^{\downarrow}_j\underline w_{ji}+x^{\uparrow}_j\overline w_{ji}\right)\rho_{\alpha^*j}\\
% &+\frac{z_i-\rho_{\alpha^*i}}{\alpha}
% \end{aligned}
% \end{equation} 
% \begin{equation}
% \label{prob:constraint2}
% x^{\leftrightarrow}_j+x^{\downarrow}_j+x^{\uparrow}_j=1,\quad \forall j\in \widehat{\mathcal{N}}_i,
% \end{equation} 
% \begin{equation}
% \label{prob:constraint3}
% w_{ji}-\lambda^*_i \rho^*_{\alpha j}\in(\underline w_{ji},\overline w_{ji}),\quad \forall j\in \widehat{\mathcal{N}}_i\,|\, x^{\leftrightarrow}_j=1,
% \end{equation} 
% \begin{equation}
% \label{prob:constraint4}
% w_{ji}-\lambda^*_i \rho^*_{\alpha j}\leq \underline w_{ji},\quad \forall j\in \widehat{\mathcal{N}}_i\,|\, x^{\downarrow}_j=1,
% \end{equation} 
% \begin{equation}
% \label{prob:constraint5}
% w_{ji}-\lambda^*_i \rho^*_{\alpha j}\geq \overline w_{ji},\quad \forall j\in \widehat{\mathcal{N}}_i\,|\, x^{\uparrow}_j=1.
% \end{equation} 
%\end{problem} 
%\vspace{2mm}
Let us first show that solving the above problem for all \mbox{$i\in\{1,\ldots,n\}$} yields a ${\bm \lambda}^*=[\lambda_1^*,\ldots,\lambda_n^*]^T$ that corresponds to the global optimal solution to Problem~\eqref{prob:convexproblem0}.
\begin{proposition}
\label{prop:closedformlambdai}
Let $\lambda^*_i\in \mathbb{R}$ and $x^{\leftrightarrow}_j,x^{\downarrow}_j,x^{\uparrow}_j \in \{0,1\}$ for all $j\in \widehat{\mathcal{N}}_i$ be a solution that satisfies the constraints in \mbox{Eqs.~\eqref{prob:constraint1}--\eqref{prob:constraint5}.}
It holds $f_i(\lambda^*_i)=0$, where $f_i(\cdot)$ is defined as in Eq.~\eqref{eq:fi}.
\end{proposition}
\begin{proof}
By using the definition of $f_i(\cdot)$ given in Eq.~\eqref{eq:fi} and by explicitly considering the sets $\widehat{\mathcal{N}}_i^{\leftrightarrow},\widehat{\mathcal{N}}_i^{\uparrow},\widehat{\mathcal{N}}_i^{\downarrow}$, we can express $f_i({ \lambda}^*_i)$ as follows
\begin{equation}
\label{eq:fispacchettata}
\begin{aligned}
f_i({ \lambda}^*_i)&= \sum_{j\in\widehat{\mathcal{N}}_i^{\leftrightarrow}}w_{ji}\rho^*_{\alpha j}-\lambda_i^* \sum_{j\in\widehat{\mathcal{N}}_i^{\leftrightarrow}}(\rho^*_{\alpha j})^2
+ \sum_{j\in\widehat{\mathcal{N}}_i^{\downarrow}} \underline w_{ji}\rho^*_{\alpha j}\\
&
+ \sum_{j\in\widehat{\mathcal{N}}_i^{\uparrow}} \overline w_{ji}\rho^*_{\alpha j}
-\frac{1}{\alpha}\rho^*_{\alpha i}+\frac{1}{\alpha}z_i=0.
\end{aligned}
\end{equation}
Since for hypothesis the variables $x^{\leftrightarrow}_j,x^{\downarrow}_j,x^{\uparrow}_j $ satisfy the constraints in Eqs.~\eqref{prob:constraint2}--\eqref{prob:constraint5}, they define consistent sets $\widehat{\mathcal{N}}_i^{\leftrightarrow},\widehat{\mathcal{N}}_i^{\uparrow},\widehat{\mathcal{N}}_i^{\downarrow}$; hence, 
we have that Eq.~\eqref{eq:fispacchettata} is equivalent to Eq.~\eqref{prob:constraint1}.
The thesis follows.
\end{proof}

The following corollaries are fundamental in order to calculate $\lambda^*_i$ in finite time.

%The following corollaries are now in order.
\begin{corollary}
\label{cor:approach0}
%Let the assumptions of Problem~\eqref{prob:convexproblem0} hold true.
The vector ${\bm \lambda}^*$ that is the stack of the solutions $\lambda^*_i$ 
%to Problem~\ref{prob:satisfaction} for all $i\in\{1,\ldots,n\}$ 
is a vector of Lagrange multipliers that satisfy the necessary and sufficient condition for Problem~\eqref{prob:convexproblem0} given in Eq.~\eqref{eq:optimallambda} of Theorem~\ref{firstorderproblema}.
\end{corollary}
\begin{proof}
The proof follows directly from Eq.~\eqref{eq:fispacchettata}. 
\end{proof}

\begin{corollary}
\label{cor:approach}
Let $x^{\leftrightarrow}_j,x^{\downarrow}_j,x^{\uparrow}_j \in \{0,1\}$ for all $j\in \widehat{\mathcal{N}}_i$ be given variables that satisfy the constraint in \mbox{Eq.~\eqref{prob:constraint2}.}
If it holds $\sum_{j\in \widehat{\mathcal{N}}_i}x^{\leftrightarrow}_j>0$, then the conditions in  Eqs.~\eqref{prob:constraint1}--\eqref{prob:constraint5}  are satisfied if and only if, choosing 
\begin{equation}
\label{lambda1}
\lambda^*_i =\frac{\alpha\displaystyle
\sum_{j\in\widehat{\mathcal{N}}_i}\left(x^{\leftrightarrow}_jw_{ji}+x^{\downarrow}_j\underline w_{ji}+x^{\uparrow}_j\overline w_{ji}\right)\rho^*_{\alpha j}+z_i-\rho^*_{\alpha i}}{\alpha\displaystyle\sum_{j\in \widehat{\mathcal{N}}_i}x^{\leftrightarrow}_j\left(\rho^*_{\alpha j}\right)^2},
\end{equation}
we have that it holds
\begin{equation}
\label{eq:verify1}
\begin{cases}
\lambda^*_i \geq \displaystyle \max_{j\in\widehat{\mathcal{N}}_i\,|\,\ x^{\downarrow}=1} \frac{w_{ji}-\underline w_{ji}}{\rho^*_{\alpha j}},\\[1.5 em]
\lambda^*_i \leq \displaystyle \min_{j\in\widehat{\mathcal{N}}_i\,|\,\ x^{\uparrow}=1} \frac{w_{ji}-\overline w_{ji}}{\rho^*_{\alpha j}},\\[1.5 em]
\lambda^*_i > \displaystyle \min_{j\in\widehat{\mathcal{N}}_i\,|\,\ x^{\leftrightarrow}=1} \frac{w_{ji}-\underline w_{ji}}{\rho^*_{\alpha j}},\\[1.5 em]
\lambda^*_i < \displaystyle \max_{j\in\widehat{\mathcal{N}}_i\,|\,\ x^{\leftrightarrow}=1} \frac{w_{ji}-\overline w_{ji}}{\rho^*_{\alpha j}}.
\end{cases}
\end{equation}

Conversely, when $\sum_{j\in \widehat{\mathcal{N}}_i}x^{\leftrightarrow}_j=0$, the conditions in  Eqs.~\eqref{prob:constraint1}--\eqref{prob:constraint5}  are satisfied if and only if
\begin{equation}
\label{eq:verify2}
\min_{j\in\widehat{\mathcal{N}}_i\,|\,\ x^{\uparrow}=1} \frac{w_{ji}-\overline w_{ji}}{\rho^*_{\alpha j}}\leq \max_{j\in\widehat{\mathcal{N}}_i\,|\,\ x^{\downarrow}=1} \frac{w_{ji}-\underline w_{ji}}{\rho^*_{\alpha j}},
\end{equation}
and
\begin{equation}
\label{checkintermedio}
\displaystyle
\sum_{j\in\widehat{\mathcal{N}}_i}\left(
%x^{\leftrightarrow}_jw_{ji}+
x^{\downarrow}_j\underline w_{ji}+x^{\uparrow}_j\overline w_{ji}\right)\rho^*_{\alpha j}+\frac{z_i-\rho^*_{\alpha i}}{\alpha}=0.
\end{equation}
In this case, the problem is solved by choosing any
\begin{equation}
\label{lambdadue}
\lambda^*_i\in\left[\displaystyle\min_{j\in\widehat{\mathcal{N}}_i\,|\,\ x^{\uparrow}=1} \frac{w_{ji}-\overline w_{ji}}{\rho^*_{\alpha j}},\,\displaystyle\max_{j\in\widehat{\mathcal{N}}_i\,|\,\ x^{\downarrow}=1} \frac{w_{ji}-\underline w_{ji}}{\rho^*_{\alpha j}}\right].
\end{equation}
\end{corollary}
\begin{proof}
The proof follows directly from  Eqs.~\eqref{prob:constraint1}--\eqref{prob:constraint5}, by explicitly considering the structure of the sets $\widehat{\mathcal{N}}_i^{\leftrightarrow},\widehat{\mathcal{N}}_i^{\downarrow},\widehat{\mathcal{N}}_i^{\uparrow}$ that correspond to the given variables $x^{\leftrightarrow}_j,x^{\downarrow}_j,x^{\uparrow}_j$.
\end{proof}
% Gabriele: itemize points
\begin{remark}
\label{Remark:finite}
A consequence of Corollaries~\ref{cor:approach0}~and~\ref{cor:approach}, is that each agent can compute $\lambda^*_i$ in finite time. Indeed, it is sufficient to enumerate all ways to partition the elements in $\widehat{\mathcal{N}}_i$ into three disjoint and possibly empty sets $\widehat{\mathcal{N}}_i^{\leftrightarrow}$, $\widehat{\mathcal{N}}_i^{\downarrow}$ and $\widehat{\mathcal{N}}_i^{\uparrow}$, and then attempt to compute a candidate solution ${ \lambda}^*_i$ following the approach in Corollary~\ref{cor:approach}. If the procedure is successful, then ${ \lambda}^*_i$ is the optimal solution, otherwise a new partition is considered until, eventually, the partition corresponding to the optimal  ${ \lambda}^*_i$ is found.
%corresponds to the solution of Problem~\ref{prob:satisfaction}. Corollary~\ref{cor:hassolution} guarantees the success of such an enumeration process.
\end{remark}


\begin{algorithm}
\caption{Proposed Algorithm to compute $\lambda^*_i$}\label{algoopt}
\begin{algorithmic}
\Procedure{OptimalLagrangeMultiplier}{}
\State\For{all $\{x^{\leftrightarrow}_j, x^{\downarrow}_j, x^{\uparrow}_j\,|\,j\in \widehat{\mathcal{N}}_i\}$ that satisfy Eq.~\eqref{prob:constraint2}}{
\State \uIf{$\sum_{j\in \widehat{\mathcal{N}}_i}x^{\leftrightarrow}_j>0$}{
\State choose $\lambda^*_i$ as in Eq.~\eqref{lambda1}
\State \If{$\lambda^*_i$ satisfies Eq.~\eqref{eq:verify1}}{
\State \Return $\lambda^*_i$
}
}
\uElseIf{Eqs.~\eqref{eq:verify2}~and~\eqref{checkintermedio} are satisfied}{
\State choose any $\lambda^*_i$ that satisfies Eq.~\eqref{lambdadue}
\State \Return $\lambda^*_i$
}
}
%\State \Return fail
\EndProcedure
\end{algorithmic}
\end{algorithm}


Algorithm~\ref{algoopt} summarizes the procedure outlined in Remark~\ref{Remark:finite}, while the next proposition 
establishes its correctness and finite-time convergence.
\begin{proposition}
Algorithm~\ref{algoopt}  is correct, i.e.,  it finds a solution $\lambda^*_i$  that satisfies $f_i(\lambda^*_i)=0$.\end{proposition}
\begin{proof}
By Proposition~\ref{prop:closedformlambdai}, it holds $f_i(\lambda^*_i)=0$ if and only if Eqs.~\eqref{prob:constraint1}--\eqref{prob:constraint5} are satisfied.
At this point we observe that, within  Algorithm~\ref{algoopt}, we enumerate all choices of variables $x^{\leftrightarrow}_j,x^{\downarrow}_j,x^{\uparrow}_j \in \{0,1\}$ that satisfy Eq.~\eqref{prob:constraint2}, and for each of these choices we follow the approach in Corollary~\ref{cor:approach} to either compute $\lambda^*_i$ or discard the choice if the conditions in Corollary~\ref{cor:approach} are not satisfied.
In conclusion, Algorithm~\ref{algoopt} correctly finds the optimal $\lambda^*_i$. 
\end{proof}
Let us now inspect the computational complexity of Algorithm~\ref{algoopt}.
\begin{proposition}
\label{prop:complex}
%Let the assumptions of Problem~\eqref{prob:convexproblem0} hold true.
Algorithm~\ref{algoopt} has a computational complexity $O(3^{|\widehat{\mathcal{N}}_i|})$.
\end{proposition}
\begin{proof}
In order to prove the statement, let us calculate the number of solutions that must be enumerated within Algorithm~\ref{algoopt}.
To this end, let us consider the Stirling numbers of the second kind  \cite{abramowitz1972stirling}, which are defined as
$$
S(n,k)=\frac{1}{k!}\sum_{j=0}^{k} (-1)^{n-j} \binom{n}{j} j^{n}
$$
and correspond to the number of {\em unordered} partitions of $n$ elements into $k$ nonempty sets (e.g., $S(3,2)=3$, since $\{x,y,z\}$ can be partitioned into sets $\{\{x\},\{y,z\}\}$, $\{\{y\},\{x,z\}\}$ or $\{\{z\},\{x,y\}\}$).
Within Algorithm~\ref{algoopt}, we enumerate all possible {\em ordered} partitions\footnote{For instance the ordered partitions of the set $\{x,y,z\}$ into two nonempty sets are six and are given by $\{\{x\},\{y,z\}\}$, $\{\{y,z\},\{x\}\}$, $\{\{y\},\{x,z\}\}$, $\{\{x,z\},\{y\}\}$, $\{\{z\},\{x,y\}\}$ and  $\{\{x,y\},\{z\}\}$.}.
We point out that, by definition, the number of ways to partition $n$ elements into $k$ nonempty ordered partitions is given by the Stirling number multiplied by the number of possible permutations of the $k$ sets, i.e., 
$$
\hat S(n,k)=k!\,S(n,k)=\sum_{j=0}^{k} (-1)^{n-j} \binom{n}{j} j^{n}.
$$
Notice that, from the definition of Stirling numbers, we have that $S(n,1)=1$, \mbox{$S(n,2)=2^{n-1}-1$} and \mbox{$S(n,3)=\frac{1}{6}(3^{n}-3\,2^{n}+3)$}; hence,
$\hat S(n,1)=1$, $\hat S(n,2)=2^{n}-2$ and \mbox{$\hat S(n,3)=3^{n}-3\,2^{n}+3$}.


At this point we observe that, since $\mathcal{G}$ is undirected and connected by hypothesis\footnote{This proposition  trivially extends to the case of a strongly connected directed graph.} it must hold $|\widehat{\mathcal{N}}_i|\geq2$.
In particular, if $|\widehat{\mathcal{N}}_i|=2$ we have to inspect a number $\nu_i$ of ordered partitions given by
$$
\nu_i=3\hat S(2,1)+3\hat S(2,2)=3+3(2^{2}-2)=9=3^{|\widehat{\mathcal{N}}_i|};
$$
in fact we can assign all the two element to each of the three sets, or we can chose any pair of sets (we have three pairs) and partition the two elements in such two sets.

Similarly, when $|\widehat{\mathcal{N}}_i|>2$ we also have the option to partition the elements into three nonempty sets, hence $\nu_i$ becomes
$$
\begin{aligned}
\nu_i&=3\hat S(|\widehat{\mathcal{N}}_i|,1)+3\hat S(|\widehat{\mathcal{N}}_i|,2)+S(|\widehat{\mathcal{N}}_i|,3)\\
&=3+3(2^{|\widehat{\mathcal{N}}_i|}-2)+3^{|\widehat{\mathcal{N}}_i|}-3\,2^{|\widehat{\mathcal{N}}_i|}+3\\
&=3^{|\widehat{\mathcal{N}}_i|}.
\end{aligned}
$$
The proof is completed by noting that, for all choices of the variables $\{x^{\leftrightarrow}_j, x^{\downarrow}_j, x^{\uparrow}_j\,|\,j\in \widehat{\mathcal{N}}_i\}$, computing $\lambda^*_i$ and checking for satisfaction of the constraints has complexity $O(1)$, as discussed in Remark~\ref{Remark:finite}.
\end{proof}

The following corollary is a consequence of the exaustive exploration of all possible partitions, which are finite and specifically amount to $3^{|\widehat{\mathcal{N}}_i|}$ as per Proposition~\ref{prop:complex}.
\begin{corollary}
Algorithm~\ref{algoopt} computes a value of $\lambda^*_i$ that satisfies $f_i(\lambda^*_i)=0$ in finite time.
\end{corollary}

Notice that the complexity of Algorithm~\ref{algoopt} is exponential in the number of neighbors of the node executing it. However, in typical applications, the neighborhood is likely to be well below the number of nodes. For instance, it can be easily shown that in random graphs (e.g., see~\cite{blum2016foundations}) the average degree is $np$, where $n$ is the number of nodes and $p$ the probability to create a link between two nodes; however, in several practical cases (e.g., while considering percolation phenomena~\cite{janson2009percolation}), we are interested in {\em sparse} random networks where $p\approx d/n$ for some fixed value $d$; hence, the average degree is $d$. Other relevant examples include lattices, where the degree is constant and typically small, and planar graphs, where the average degree is upper bounded by six (see, for instance, \cite{nishizeki1988planar}). 

==> asymptotic.tex <==
\section{Asymptotic Distributed Algorithm in Continuous Time}
We now show that the algorithm
\begin{equation}
\label{eq:algocontinuous}
\dot {\bm \lambda}(t)=\left(\alpha\mathbf{Z}^T({\bm \lambda}(t))-\mathbf{I}_n\right)\bm\rho_\alpha^*+\mathbf{z}
\end{equation}
converges to a ${\bm \lambda}^{eq}$ that satisfies the condition in Eq.~\eqref{eq:optimallambda}.
\textcolor{red}{NOTE: each equation can be solved by an agent without cooperating with the others.}
To this end, we first review the basics of nonsmooth analysis, then we demonstrate convergence of the proposed algorithm.
\subsection{Nonsmooth Analysis} \label{sec:nonsmooth}
In this subsection, we review the Filippov solution concept for differential equations with discontinuous right-hand side, the nonsmooth analysis of Clarke's Generalized Gradient, the chain-rule for differentiating regular functions along Filippov solution trajectories, and a nonsmooth version of the LaSalle's stability theorem. The reader is referred to \cite{Paden:1987,Paden:1994,Cortes:2008} and references therein for a comprehensive overview of the topic. 
Let us consider the differential equation
%
\begin{equation} \label{eq:discontinuous:equation}
%\dot {\bm x} =  f({\bm x}), \textcolor{red}{  \dot {\bm x}(t) =  f({\bm x}(t)),}
\dot {\bm x}(t) =  f({\bm x}(t)),
\end{equation}
%
with $f(\cdot) \,:\, \mathbb{R}^n \rightarrow \mathbb{R}^n$ a measurable and essentially locally bounded function. In the following, where understood, we omit the time-dependency for the sake of clarity. First, we need to clarify what it means to be a solution of this equation.
\begin{definition}[Filippov Solution]
A vector function  ${\bm x}(\cdot)$ is called solution of Eq.~\eqref{eq:discontinuous:equation} on a time interval $[t_0, \, t_i]$ if ${\bm x}(\cdot)$ is absolutely continuous on $[t_0, \, t_i]$ and for almost all $t \in [t_0, \, t_i]$ it holds \mbox{$\dot {\bm x} \in K[{\bm f}]({\bm x})$}, with $K[{\bm f}]({\bm x}) : \mathbb{R}^n \rightarrow 2^{\mathbb{R}^n}$ defined as follows
%
\begin{equation*}
K[{\bm f}]({\bm x}) \equiv \bigcap_{\delta > 0} \bigcap_{\mu\{H\} = 0} \cco \{ {\bm f} (B({\bm x},\delta) \setminus H )\}, 
\end{equation*}
%
where $ \bigcap_{\mu\{H\} = 0}$ denotes the intersection over all sets $H$ of Lebesgue  measure zero, $B({\bm x},\delta)$ denotes the ball of radius $\delta$ centered at ${\bm x}$,  $\cco$ the convex closure and $2^{\mathbb{R}^n}$ the set of subsets of $\mathbb{R}^n$.
\end{definition}
%
Briefly, the idea of the Filippov's solution is that the tangent vector to a solution, where it exists, must lie in the convex closure of the values of the vector field in progressively smaller neighborhoods around the solution point. A very important  aspect of this definition is given by the possibility of discarding sets of measure zero. Indeed, this technical detail allows solutions to be defined even at points where the vector field itself is not defined. 
We now review the concept of Clarke's Generalized Gradient.%, an essential tool in the machinery of nonsmooth analysis.
\begin{definition}[Clarke's Generalized Gradient]
Consider  a locally Lipschitz function $V \, :  \, \mathbb{R}^n \rightarrow \mathbb{R}$. Then, the generalized gradient at ${\bm x}$ is defined as
%
\begin{equation*}
\partial_{\bm x} V ({\bm x})  = \cco \left \{ \lim_{i \rightarrow \infty} \nabla V_{\bm x} ({\bm x}_i)  \, | \, {\bm x}_i \rightarrow {\bm x}, \, {\bm x}_i \notin \Omega_V \right \},
\end{equation*}
%
where $\Omega_V$ is the set of measure zeros where the gradient of $V$ is not defined.
\end{definition}
%
We now review the chain rule which allows to differentiate Lipschitz regular functions along the Filippov's solution trajectories.
\begin{theorem}[Chain Rule~{\cite{Paden:1994}}] \label{th:chain:1}
Let ${\bm x}(\cdot)$ be a Filippov solution to Eq.~\eqref{eq:discontinuous:equation} on an interval containing $t$ and $V \, : \, \mathbb{R}^n \rightarrow \mathbb{R}$ be a Lipschitz and, in addition, regular function. Then $V({\bm x})$ is absolutely continuous, $(d/dt) V({\bm x}(t))$ exists almost everywhere and
\mbox{
$
\frac{d}{dt} V({\bm x}(t)) \in^{\text{a.e.}} \dot{\widetilde{V}}({\bm x}(t)),
$}
%
where the generalized time derivative $\dot{\widetilde{V}}({\bm x})$ is defined as
%
\mbox{
$
\dot{\widetilde{V}}({\bm x}) := \bigcap_{{\bm \xi} \in \partial_{{\bm x}} V({\bm x})} \, {\bm \xi}^T K[{\bm f}]({\bm x})
$}.
\end{theorem}
%
We now review a nonsmooth version of LaSalle's Theorem~{\cite{Paden:1994}}.  This will prove useful to demonstrate the convergence of the proposed algorithm to the optimal solution of Problem~RP1.
\begin{theorem}[Nonsmooth LaSalle Theorem] \label{th:lasalle}%Invariance Principle
Let $\Omega$ be a compact set such that every Filippov solution to~\eqref{eq:discontinuous:equation} starting in $\Omega$ is unique and remains in $\Omega$ for all $t\geq0$. Let $V \, : \, \Omega \rightarrow \mathbb{R}$ be a time independent regular function such that ${\bm v} \leq 0$ for all ${\bm v} \in \dot{\widetilde{V}}({\bm x})$ (if $\dot{\widetilde{V}}({\bm x})$ is the empty set then this is trivially satisfied). Define $S = \{ {\bm x} \in \Omega \, : \, {\bm 0}_n \in \dot{\widetilde{V}}({\bm x}) \}$. Then every trajectory in $\Omega$ converges to the largest invariant set $M$, in the closure of $S$.
\end{theorem}
%
Finally, we  review  a calculus for computing the Filippov's differential inclusions, originally developed in~\cite{Paden:1987} (and further extended in~\cite{Cortes:2008}). 
%
\begin{theorem}[Calculus for K]%~{\cite{Paden:1987}}]
\label{th:calculus}
Let us consider the map \mbox{$K:\mathbb{R}^n \rightarrow 2^{\mathbb{R}^n}$}; $K$ has the following properties.
%
\begin{enumerate}
\item Assume that ${\bm f} \, : \, \mathbb{R}^n \rightarrow \mathbb{R}^n$ is locally bounded. Then $\exists \, H_{{\bm f}} \subset \mathbb{R}^n, \, \mu\{ H_{{\bm f}}\}=0$, such that $\forall \, { H}  \subset \mathbb{R}^n$, \mbox{$\mu \{{H}\}=0$,}
%
\begin{equation*}
K[{\bm f}]({\bm x}) = \co \left \{ \lim_{i \rightarrow \infty} f({\bm x}_i) \, | \,  {\bm x}_i \rightarrow {\bm x}, {\bm x}_i   \notin H_{{\bm f}} \bigcup {H} \right \}. 
\end{equation*}
\item Assume that ${\bm f}, \, {\bm g}: \mathbb{R}^n \rightarrow \mathbb{R}^n$ are locally bounded; then
\mbox{$
K[{\bm f}+{\bm g}]({\bm x}) \subset K[{\bm f}]({\bm x}) + K[{\bm g}]({\bm x}).
$}
\item Assume that $f_i \, : \, \mathbb{R}^n \rightarrow \mathbb{R}^{n_i}, \, j \in \{1, \, \ldots, \, N \}$, are locally bounded; then
\begin{equation*}
%K \left [  \mathlarger{\mathlarger{\times}}_{j=1}^N f_j ({\bm x}) \right ] \subset  \mathlarger{\mathlarger{\times}}_{j=1}^N K[f_j]({\bm x}),
K \left [  \bigtimes_{j=1}^N f_j ({\bm x}) \right ] \subset \bigtimes_{j=1}^N K[f_j]({\bm x}),
\end{equation*}
where the cartesian product notation and the column vector notation are used interchangeably.
\item Let ${\bm g} \, : \, \mathbb{R}^m \rightarrow \mathbb{R}^{p \times n}$ (i.e., matrix valued) be continuous  and ${\bm f} \, : \, \mathbb{R}^m \rightarrow \mathbb{R}^n$ be locally bounded; then
\mbox{$
K[{\bm g} \, {\bm f}]({\bm x}) = {\bm g}({\bm x}) \, K[{\bm f}]({\bm x}),
$}
%
where  ${\bm g}\,{\bm f} \triangleq {\bm g}({\bm x}) \, {\bm f}({\bm x}) \in \mathbb{R}^p$.
\item Let $V: \, \mathbb{R}^n  \rightarrow \mathbb{R}$ be locally Lipschitz continuous; then 
\mbox{$
\partial_{{\bm x}} V ({\bm x}) = K [\nabla V] ({\bm x}).
$}
%
\item Let ${\bm f}:\mathbb{R}^n \rightarrow \mathbb{R}^n$ be continuous; then it holds
\mbox{$
K[{\bm f}]({\bm x}) = \{ {\bm f}({\bm x}) \}.
$}
\end{enumerate}
\end{theorem}
%
\begin{theorem}
The Algorithm in Eq.~\eqref{eq:algocontinuous} coonverges to a $ {\bm \lambda}^{eq}$ such that the necessary and sufficient optimality condition in Eq.~\eqref{eq:optimallambda} is satisfied. Moreover, by Eq.~\ref{eq:optimallambda}, it holds $\lim_{t\rightarrow \infty} \mathbf{X}(t)=\mathbf{X}^*$.
\end{theorem}
\begin{proof}
We now demonstrate the convergence properties of the proposed algorithm.
To this end, we note that
%
\begin{equation}
\nabla_{\lambda_h} z_{ij}(\cdot) = 
\begin{cases}
-\rho_{\alpha^*i} & \text{if } h=j \mbox{ and } w_{ij}-\lambda_j\rho_{\alpha^*i}\in (\underline w_{ij}, \, \overline w_{ij}) \\[5pt]
0 & \text{if } h\neq j \mbox{ or }  w_{ij}-\lambda_j\rho_{\alpha^*i} < \underline w_{ij}  \\
&\mbox{ or } w_{ij}-\lambda_j\rho_{\alpha^*i} > \overline w_{ij}
\end{cases}
\end{equation}
%
and the related Filippov map $K [ \nabla_{\lambda_h} z_{ij}(\cdot)]$ is defined as follows
%
\begin{equation}
K [\nabla_{\lambda_h} {z}_{ij}(\cdot)]=
\begin{cases}
%\left \{ \nabla_x \sigma(x, a, b) \right \} & \text{if }  x \neq a \, \land x \neq b \\ 
\{ -\rho_{\alpha^*i} \} & \text{if } h=j \\
&\mbox{ and } w_{ij}-\lambda_j\rho_{\alpha^*i}\in (\underline w_{ij}, \, \overline w_{ij}) \\[5pt]
\cco \{-\rho_{\alpha^*i}, \, 0\} & \text{if } h=j \\
&\mbox{ and } w_{ij}-\lambda_j\rho_{\alpha^*i}\in \{\underline w_{ij}, \, \overline w_{ij}\}\\[5pt]
\{ 0 \} & \text{ otherwise}. \\
\end{cases}
\end{equation}
%
Let us denote by $\mathbb{L}$ the matrix valued set such that
$\mathbb{L}_{ij}=K [\nabla_{\lambda_j} {z}_{ij}(\cdot)]$.
%
We now characterize the Filippov map  $K[ \nabla_{\bm \lambda}  f({\bm \lambda}) ]$ for the $n\times n$ Jacobian matrix $\nabla_{\bm \lambda} f({\bm \lambda})$ of the vectorial function \mbox{$f({\bm \lambda})=\left(\alpha\mathbf{Z}^T({\bm \lambda})-\mathbf{I}_n\right)\bm\rho_\alpha^*+\mathbf{z}$} with respect to ${\bm \lambda}$.
To this end, we notice that, by using the Property~$3$ of the Filippov Calculus,  it holds
\mbox{$K[ \nabla_{\bm \lambda}  f({\bm \lambda})]\subset \mathbb{K}$,}
where $\mathbb{K}$ is the $n\times n$ matrix-valued set such that $\mathbb{K}_{ij}=K \left [  \nabla_{ \lambda_j}  f_i({\bm \lambda}) \right ]$, for all \mbox{$i,j\in\{1,\ldots,n\}$}
%
At this point we note that it holds
\begin{equation} \label{eq:partial_w:1}
K \left [  \nabla_{ \lambda_j}  f_i({\bm \lambda}) \right ] \subset
\begin{cases}
\sum_{h \in \mathcal{N}_i} K [\nabla_{\lambda_i} {z}_{ih}(\cdot)]& \text{if } i=j \\[5pt]
\left \{ 0 \right \} & \text{otherwise},
\end{cases}
\end{equation}
%
To summarize, we have that 
$$K[ \nabla_{\bm \lambda}  f({\bm \lambda})]\subset \mathbb{K}',$$
where $\mathbb{K}'$ is the set of all matrices $\Xi'\in \mathbb{R}^{n\times n}$ with
%
$$
\Xi'=\Delta(L{\bm 1}_n), \quad L\in \mathbb{L}.
$$
%
Notice that, by construction, all $\Xi'\in\mathbb{K}'$ are diagonal and negative semidefinite.

We are now in position to prove convergence of the proposed algorithm.

Let us consider the candidate Lyapunov function 
$$
V({\bm \lambda})=\|{\bm f}({\bm \lambda})\|^2/2
$$
which clearly satisfies $V({\bm \lambda})>0$, for all ${\bm \lambda}\neq {\bm 0}_n$ and, since it holds $\underline w_{ij}\leq w_{ij}\leq\overline w_{ij}$ we have that ${\bm f}({\bm 0}_n)={\bm 0}_n$ and $V({\bm 0}_{n})=0$.
The generalized derivative $\dot{\widetilde{V}}({\bm \lambda})$ is such that 
%
\mbox{$
%\begin{aligned}
\dot{\widetilde{V}}({\bm \lambda})= \bigcap_{{\bm \xi}\in \partial_{{\bm \lambda}} V({\bm \lambda})} \, {\bm \xi}^T K[f({\bm \lambda})]
%\end{aligned}
$}
%
where in our case $\partial_{{\bm \lambda}} V({\bm \lambda})$ takes the form:
%
\begin{equation} \label{eq:supp_lyap:1}
\partial_{{\bm \lambda}} V({\bm \lambda}) = f^T({\bm \lambda}) \, K \left [ \nabla_{\bm \lambda} f^T({\bm \lambda}) \right ],
\end{equation}
%
while
\begin{equation}  \label{eq:supp_lyap:2}
K[f^T({\bm \lambda})] = \{ f^T({\bm \lambda})\}
\end{equation}
%
being $f^T({\bm \lambda})$ continuous.  We observe that by construction each ${\bm \xi} \in \partial_{{\bm \lambda}} V({\bm \lambda})$ has the form
%
\begin{equation}  \label{eq:supp_lyap:3}
{\bm \xi} = f^T({\bm \lambda}) \, {\bm \Xi}, \quad   {\bm \Xi} \in K \left [ \nabla_{\bm \lambda} f^T({\bm \lambda}) \right ].
\end{equation}
%
Now, by putting Eqs.~\eqref{eq:supp_lyap:1},~\eqref{eq:supp_lyap:2} and~\eqref{eq:supp_lyap:3} together we obtain
%
\begin{equation*}
\begin{aligned}
\dot{\widetilde{V}}({\bm \lambda}) &= \bigcap_{ {\bm \Xi} \in K \left [ \nabla_{\bm \lambda} f({\bm \lambda}) \right ]} \, 
f^T({\bm \lambda}) \, {\bm \Xi}  \, f({\bm \lambda})
\end{aligned}
\end{equation*}
%
At this point, since any $\Xi$ satisfies 
$$\Xi \in K \left [ \nabla_{\bm \lambda} f({\bm \lambda}) \right ]\subset\mathbb{K}',$$
we have that $\Xi$ is negative semidefinite. 
To demonstrate the convergence of our algorithm, we invoke the nonsmooth version of the Lasalle invariance principle detailed in Theorem~\ref{th:lasalle}. In particular,  we consider the set \mbox{$S=\{
{\bm \lambda}\in \mathbb{R}^{n}\,|\, \dot{\widetilde V}({\bm \lambda})=0
\}$}, which can be expressed as \mbox{$S=
\left\{
{\bm \lambda}\in \mathbb{R}^{n}\,|\,  f(\cdot) \in \ker \left (  {\bm \Xi} \right )\right., \left. {\bm \Xi} \in  K \left [ \nabla_{\bm \lambda} f(\cdot) \right ]
\right\}.$}
%\begin{equation*}
%\begin{aligned}
%S&=
%\left\{
%{\bm \lambda}\in \mathbb{R}^{n}\,\Big|\,  f(\cdot) \in \ker \left (  {\bm \Xi} \right )\right., \left. {\bm \Xi} \in  K \left [ \nabla_{\bm \lambda} f(\cdot) \right ]
%\right\}.
%\end{aligned}
%\end{equation*}
%
From the nonsmooth version of the LaSalle's invariance principle given in Theorem~\ref{th:lasalle}, we know that every trajectory converges to the largest invariant set $M$  is contained in the closure of the $S$.  In particular, we notice that  for any given ${\bm \lambda}$ such that $f({\bm \lambda}) \in \ker \left (  {\bm \Xi} \right )$ with $f({\bm \lambda}) \neq {\bm 0}_n$, it follows that  $\dot {\bm \lambda}(\bar t)\neq0$, therefore $f({\bm \lambda})$ cannot stay  in $\ker \left (  {\bm \Xi} \right )$, and thus the solution leaves the set $S$. It follows that the only  ${\bm \lambda}$ such that the solutions stay in the  $S$ are those such that  $f({\bm \lambda}) = {\bm 0}_{n}$ for which $\dot {\bm \lambda}(\bar t) = 0$, that is we can define the largest invariant set as
\mbox{$M=\{ {\bm \lambda}^*\in \mathbb{R}^{n}\,|\, f(\cdot)={\bm 0}_{n}\}$}.
Therefore, we conclude that by running the algorithm in Eq.~\eqref{eq:algocontinuous} we asymptotically compute a $ {\bm \lambda}^{eq}$ such that the necessary and sufficient optimality condition in Eq.~\eqref{eq:optimallambda} is satisfied. Moreover, by Eq.~\ref{eq:optimallambda}, it holds $\lim_{t\rightarrow \infty} \mathbf{X}(t)=\mathbf{X}^*$.
The thesis follows.
\end{proof}

\section{Asymptotic Distributed Algorithm in Discrete Time}
Let $\theta\in\mathbb{R}_{>0}$, $\theta<(\max_{i=1,\ldots,n}\{|\hat{\mathcal{N}}_i|\})^{-1}$.
We now show that the algorithm
\begin{equation}
\label{eq:algodiscrete}
{\bm \lambda}(k+1)={\bm \lambda}(k)+\theta\left(\alpha\mathbf{Z}^T({\bm \lambda}(k))-\mathbf{I}_n\right)\bm\rho_\alpha^*+\theta\mathbf{z}
\end{equation}
converges to a ${\bm \lambda}^{eq}$ that satisfies the condition in Eq.~\eqref{eq:optimallambda}.
\textcolor{red}{NOTE: each equation can be solved by an agent without cooperating with the others.}
\subsection{Proof of Convergence}
